Passive inverse obstacle scattering problems for the Helmholtz equation

Passive imaging involves recording waves generated by uncontrolled, random sources and utilizing correlations of such waves to image the medium through which they propagate. In this paper, we focus on passive inverse obstacle scattering problems governed by the Helmholtz equation in $\mathbb{R}^d\;(d=2,3)$. The random source is modelled by a Gaussian random process. Uniqueness results are established for the inverse problems to determine the source strength or shape and location of an obstacle, or both of them simultaneously from near-field correlation measurements. Finally, we present efficient methods for numerical reconstructions.

==> Dir-source-obstacle/source_obstacle.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=1.5in,
height=1.5in,
at={(0.867in,0.478in)},
scale only axis,
point meta min=0.503394093449599,
point meta max=13.2192152128964,
axis on top,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=-3,
xmax=3,
xtick={-3,-1.5,0,1.5,3},
tick align=outside,
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymin=-3,
ymax=4,
ytick={-3,-1.5,0,1.5,3},
axis background/.style={fill=white},
title style={font=\normalfont},
title={Source and obstacle},
%legend style={legend cell align=left, align=left, draw=black},
legend style={legend cell align=left, align=left, draw=black, font=\tiny, at={(1,0.7)}, anchor=south east},
colormap/hot2,
colorbar,
colorbar style={separate axis lines, every outer x axis line/.append style={black}, every x tick label/.append style={font=\color{black}}, every x tick/.append style={black}, every outer y axis line/.append style={black}, every y tick label/.append style={font=\color{black}}, every y tick/.append style={black}}
]
\addplot [forget plot] graphics [xmin=-2.03571428571429, xmax=-1.46428571428571, ymin=-1.54838709677419, ymax=1.54838709677419] {Dir-source-obstacle/source_obstacle-1.png};
\addplot [forget plot] graphics [xmin=1.46428571428571, xmax=2.03571428571429, ymin=-1.54838709677419, ymax=1.54838709677419] {Dir-source-obstacle/source_obstacle-2.png};
\addplot [color=orange, line width=1.5pt]
  table[row sep=crcr]{%
-0.149941639973572	0.501048116788004\\
-0.133843792338541	0.385289063835608\\
-0.0782051586544083	0.285974456291364\\
0.00722405612213784	0.194905919934387\\
0.10925366094537	0.110155104148614\\
0.218262542944971	0.0253720236725542\\
0.321080681214414	-0.0622345919890673\\
0.408338203540294	-0.158482280925378\\
0.466486393236096	-0.266325371693579\\
0.505157952343543	-0.385070062146835\\
0.538901652772338	-0.509333132855938\\
0.564298688438677	-0.638037232380894\\
0.578823283965763	-0.766742534451507\\
0.579268435191686	-0.894061628627929\\
0.562682703126582	-1.01569820861145\\
0.526309907313376	-1.13001183469485\\
0.465253860278564	-1.23494145972515\\
0.362134329376925	-1.34942174423232\\
0.225447661988721	-1.4617038746279\\
0.0694442188187118	-1.56137837656411\\
-0.0966477333142413	-1.63925592924197\\
-0.260348114558843	-1.68796404184409\\
-0.412263147945908	-1.69707752697889\\
-0.53968102831698	-1.66037054665443\\
-0.632718016899188	-1.56753549331994\\
-0.652966052607406	-1.4613858193447\\
-0.591792094332252	-1.37322447216791\\
-0.475362387336835	-1.2932747254772\\
-0.325433902911742	-1.21796047021955\\
-0.166427950832406	-1.13985271764912\\
-0.0212772984721446	-1.0538685255848\\
0.0865926193416984	-0.953641729425033\\
0.133275065456301	-0.83437878345467\\
0.117177063721951	-0.718619730502275\\
0.0615384745660109	-0.619305122958031\\
-0.023890767241255	-0.528236586601054\\
-0.125920352259196	-0.44348577081528\\
-0.234929250225721	-0.358702690339221\\
-0.337747374773873	-0.271096074677599\\
-0.42500490952233	-0.174848385741289\\
-0.483153087389525	-0.0670052949730876\\
-0.521824658397032	0.0517393954801681\\
-0.555568346176246	0.176002466189271\\
-0.580965393134846	0.304706565714227\\
-0.59548969932216	0.43341186778484\\
-0.595934789755774	0.560730961961262\\
-0.579349076083284	0.682367541944783\\
-0.542976269726607	0.796681168028183\\
-0.48192023028051	0.901610793058486\\
-0.378800693156139	1.01609107756565\\
-0.242114031338956	1.12837320796124\\
-0.0861105828573844	1.22804770989744\\
0.0799813639709613	1.3059252625753\\
0.243681750702025	1.35463337517742\\
0.3955967782568	1.36374686031223\\
0.523014664970328	1.32703987998776\\
0.616051646513042	1.23420482665328\\
0.636299690193864	1.12805515267803\\
0.575125722686913	1.03989380550124\\
0.458696026672357	0.959944058810537\\
0.308767528710407	0.884629803552878\\
0.149761594220362	0.806522050982455\\
0.00461091690170424	0.720537858918135\\
-0.103258958367591	0.620311062758366\\
-0.149941639973572	0.501048116788004\\
};
\addlegendentry{True curve}

\addplot [color=gray, line width=1.5pt]
  table[row sep=crcr]{%
0.0122733072808549	-1.61494779786161\\
0.0753045470308661	-1.6068993320227\\
0.13230643890902	-1.57881910216084\\
0.178114084238647	-1.53478077094656\\
0.21271103218874	-1.48148193250404\\
0.237391544386995	-1.42292779256146\\
0.255494609943319	-1.36201807244844\\
0.270106140467747	-1.30017780916862\\
0.282473285820075	-1.23784989645996\\
0.293147644227852	-1.17520986884689\\
0.301956468937787	-1.11228038772705\\
0.310243540005395	-1.04928007471272\\
0.318893506602123	-0.986328561111699\\
0.32712708542956	-0.923321234819625\\
0.334301111640158	-0.860184491676562\\
0.340544413836571	-0.796948930759719\\
0.346200735964044	-0.733658165187056\\
0.351384457143519	-0.670326940490885\\
0.355998556116153	-0.606951668677233\\
0.359907849201983	-0.543529019612782\\
0.3630517663736	-0.480063826226159\\
0.365527682236251	-0.416569064021513\\
0.367461443792031	-0.35305547844308\\
0.368833873790785	-0.289527284523514\\
0.369527235084287	-0.225988050684096\\
0.369447803971991	-0.162445083508477\\
0.368549645843299	-0.0989084145781705\\
0.366872865908379	-0.0353875251335686\\
0.364572287409382	0.0281138317444811\\
0.361827147941891	0.0915975241078551\\
0.358658712376831	0.155061498162854\\
0.354880228865579	0.218492074773339\\
0.350342032407699	0.281872827054242\\
0.345086557702587	0.345198137731786\\
0.338825400569547	0.408431933269764\\
0.331034194169084	0.471495489224126\\
0.32228432065416	0.534433194141419\\
0.31389086805082	0.597419422320117\\
0.30608798673441	0.660481534796195\\
0.297095789388963	0.723385075027918\\
0.28499350478361	0.785764957154406\\
0.271600729340809	0.847880563508383\\
0.260520151431765	0.910450011164448\\
0.246985025648622	0.972534754514308\\
0.226991447866291	1.03285035642828\\
0.210393619084698	1.09418735233223\\
0.185690977221306	1.15273215971728\\
0.149915815174163	1.20524742194917\\
0.104564193470371	1.24975523469726\\
0.0484488175748869	1.27956764108944\\
-0.0146196797704756	1.28731874613204\\
-0.0758791144547647	1.27043690236589\\
-0.128302370032466	1.23452705327934\\
-0.168828256018908	1.18558456098688\\
-0.199507585310063	1.12993841340209\\
-0.221444047649195	1.07030195972795\\
-0.238828896945421	1.00918337007038\\
-0.25330992400194	0.947312416932645\\
-0.266786903330837	0.885215025562701\\
-0.282177891965121	0.823564133795891\\
-0.295917641549925	0.761524354072472\\
-0.305013622280037	0.6986357372858\\
-0.310981650588287	0.635373603075078\\
-0.31745459532257	0.572161136161894\\
-0.326287942035999	0.509235092486609\\
-0.33631734748428	0.446488570565968\\
-0.345119659992099	0.383558178216181\\
-0.351150669700464	0.320302017182799\\
-0.35478561697595	0.256863053248259\\
-0.357653778003587	0.193384799971227\\
-0.360792278580292	0.129919338490879\\
-0.364097592024437	0.0664623460486003\\
-0.36709916248155	0.00299026114842968\\
-0.369343450477018	-0.0605131100863078\\
-0.370479982397387	-0.124045962076262\\
-0.370478240197162	-0.187588978873926\\
-0.369659948389828	-0.2511267265937\\
-0.368566466903158	-0.314660334117763\\
-0.367382470802894	-0.37819231929073\\
-0.365819321962486	-0.441716106587193\\
-0.363229797037992	-0.505206336917921\\
-0.359223336691215	-0.568622921990543\\
-0.354345737191754	-0.631978458527663\\
-0.349412010872846	-0.695329648977359\\
-0.344373669112038	-0.75867260516891\\
-0.338591695013489	-0.821952015424594\\
-0.331802737950302	-0.885131324132253\\
-0.324034367375478	-0.948197697148273\\
-0.315622551819222	-1.01118147558233\\
-0.307033669133691	-1.07414135233728\\
-0.298359144115146	-1.13708948656289\\
-0.289193262704417	-1.19996795350308\\
-0.27959849200064	-1.26278240535873\\
-0.264804293551827	-1.32457922306838\\
-0.247752248288461	-1.38579149911755\\
-0.227405610799124	-1.44598891874382\\
-0.20064784656047	-1.5036234313186\\
-0.160803046236957	-1.55312198557994\\
-0.111214418980975	-1.59285463001308\\
-0.0512612350298965	-1.61391005023951\\
0.0122733072808549	-1.61494779786161\\
};
\addlegendentry{Initial guess}

\addplot [color=black, line width=1.5pt]
  table[row sep=crcr]{%
-0.01212176797959	-1.59135549390472\\
0.131328384473133	-1.52909714859957\\
0.209366267547275	-1.478451247256\\
0.266497733113169	-1.43155129076354\\
0.316554546109299	-1.38784061169924\\
0.362826401985645	-1.34515369008436\\
0.401395076049752	-1.30943332294881\\
0.436691748111024	-1.2757617058347\\
0.466425701487267	-1.24329893697275\\
0.494306186370704	-1.20643575200157\\
0.519654201828462	-1.16435710428187\\
0.541939045888149	-1.1146946845021\\
0.558291151236879	-1.05965265268586\\
0.56763657479354	-1.00014740683823\\
0.571987204595241	-0.937551256103994\\
0.572888758811173	-0.86717890476426\\
0.571565174963302	-0.789615041112515\\
0.569699501191711	-0.708720592232807\\
0.566637895826832	-0.63103561271228\\
0.560164701923147	-0.557596502942403\\
0.546766834482386	-0.483289897577715\\
0.522925844809119	-0.406565841606577\\
0.482937128619294	-0.323509445610293\\
0.432232022594818	-0.244537920634498\\
0.374332281234297	-0.163077835135162\\
0.319643468236336	-0.0845564845622068\\
0.260787753500806	-0.00134299717324354\\
0.202757364774712	0.0755271750712775\\
0.13841155712615	0.15308552187187\\
0.0804210833995567	0.221289861904785\\
0.0237124204626953	0.291878954132816\\
-0.0204000640092279	0.356619439257687\\
-0.0578642940203471	0.429327906324743\\
-0.0802344681384652	0.499552340361726\\
-0.0888513727745981	0.576231752913194\\
-0.0814484406618553	0.647889631902096\\
-0.0564100626701971	0.722774903563838\\
-0.0107627736145724	0.793849715167374\\
0.0500286588564666	0.84961332174843\\
0.118955207149568	0.889164002543469\\
0.179014681172433	0.912957619868527\\
0.248027256293638	0.931992993109546\\
0.304339668642678	0.941135690663474\\
0.37431704075928	0.950606359583554\\
0.420322859118152	0.956311778499767\\
0.485173650512491	0.966537153008597\\
0.532169750486135	0.983712685614542\\
0.62520270556879	1.07255676777281\\
0.626108812932464	1.1426420106266\\
0.623936732477639	1.14965599067782\\
0.617284607744659	1.16581167564338\\
0.544364365732897	1.31477807837924\\
0.176541524787411	1.35899696938213\\
0.108499602210057	1.30913313246204\\
0.0451156925908899	1.23765268688071\\
-0.0253732676615592	1.19166940435503\\
-0.114902140955695	1.17958374228294\\
-0.191454245201484	1.18420172799584\\
-0.255482217011852	1.17019791993787\\
-0.308359064405514	1.11276868206274\\
-0.332934421757953	1.03405164775077\\
-0.356630582412156	0.967836405804628\\
-0.413876477938651	0.898602775188868\\
-0.476486211724799	0.85650980607126\\
-0.518058122887598	0.833046467723274\\
-0.558677945441327	0.798176944647571\\
-0.59211851051255	0.729631932574944\\
-0.603638351027961	0.64152531927689\\
-0.598198514633337	0.517988004031367\\
-0.589142460869137	0.406286599452341\\
-0.568812519789944	0.275079329496299\\
-0.545832942974299	0.142976186530931\\
-0.511701881472895	0.00274327068882237\\
-0.465606283376003	-0.116877733399806\\
-0.39444061872867	-0.220661005969353\\
-0.313800417158799	-0.297672528009224\\
-0.231410616171428	-0.366372185340484\\
-0.151631637663082	-0.434912925748525\\
-0.0697877713824945	-0.514219140469202\\
-0.000744878144324362	-0.59527381416607\\
0.0528434325400872	-0.680588568100819\\
0.0843971285031483	-0.767103458797708\\
0.093175420764861	-0.856712635306531\\
0.0784176510600476	-0.944981774767809\\
0.0419305858967867	-1.02288469690719\\
-0.0164479438731146	-1.09098167396912\\
-0.0964957363578005	-1.1455923535824\\
-0.201282269634396	-1.19144373741583\\
-0.320670034244806	-1.23002225131467\\
-0.430501449327456	-1.26636198605695\\
-0.528044594601867	-1.31059596242992\\
-0.597448262417165	-1.37038437755243\\
-0.649078417489811	-1.48315813447669\\
-0.635829800683342	-1.57592127114574\\
-0.557057233478389	-1.64773979703646\\
-0.459365234290085	-1.68839757023748\\
-0.342680974888292	-1.71171740633952\\
-0.236950333905388	-1.67975406589511\\
-0.186162460668174	-1.65460161864113\\
-0.128328233032891	-1.62691509019931\\
-0.01212176797959	-1.59135549390472\\
};
\addlegendentry{Reconstruction}

\end{axis}
\end{tikzpicture}%

==> Dir-source-obstacle/source_obstacle4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width = 1.5in,
height = 1.5in,
at={(0.867in,0.478in)},
scale only axis,
point meta min=0.384130906386258,
point meta max=12.753944382351,
axis on top,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=-3,
xmax=3,
xtick={-3,-1.5,0,1.5,3},
tick align=outside,
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymin=-3,
ymax=4,
ytick={-3,-1.5,0,1.5,3},
axis background/.style={fill=white},
title style={font=\normalfont},
title={Source and obstacle},
%legend style={legend cell align=left, align=left, draw=black},
legend style={legend cell align=left, align=left, draw=black, font=\tiny, at={(1,0.7)}, anchor=south east},
colormap/hot2,
colorbar,
colorbar style={separate axis lines, every outer x axis line/.append style={black}, every x tick label/.append style={font=\color{black}}, every x tick/.append style={black}, every outer y axis line/.append style={black}, every y tick label/.append style={font=\color{black}}, every y tick/.append style={black}}
]
\addplot [forget plot] graphics [xmin=-2.03571428571429, xmax=-1.46428571428571, ymin=-1.54838709677419, ymax=1.54838709677419] {Dir-source-obstacle/source_obstacle4-1.png};
\addplot [forget plot] graphics [xmin=1.46428571428571, xmax=2.03571428571429, ymin=-1.54838709677419, ymax=1.54838709677419] {Dir-source-obstacle/source_obstacle4-2.png};
\addplot [color=orange, line width=1.5pt]
  table[row sep=crcr]{%
-0.149941639973572	0.501048116788004\\
-0.133843792338541	0.385289063835608\\
-0.0782051586544083	0.285974456291364\\
0.00722405612213784	0.194905919934387\\
0.10925366094537	0.110155104148614\\
0.218262542944971	0.0253720236725542\\
0.321080681214414	-0.0622345919890673\\
0.408338203540294	-0.158482280925378\\
0.466486393236096	-0.266325371693579\\
0.505157952343543	-0.385070062146835\\
0.538901652772338	-0.509333132855938\\
0.564298688438677	-0.638037232380894\\
0.578823283965763	-0.766742534451507\\
0.579268435191686	-0.894061628627929\\
0.562682703126582	-1.01569820861145\\
0.526309907313376	-1.13001183469485\\
0.465253860278564	-1.23494145972515\\
0.362134329376925	-1.34942174423232\\
0.225447661988721	-1.4617038746279\\
0.0694442188187118	-1.56137837656411\\
-0.0966477333142413	-1.63925592924197\\
-0.260348114558843	-1.68796404184409\\
-0.412263147945908	-1.69707752697889\\
-0.53968102831698	-1.66037054665443\\
-0.632718016899188	-1.56753549331994\\
-0.652966052607406	-1.4613858193447\\
-0.591792094332252	-1.37322447216791\\
-0.475362387336835	-1.2932747254772\\
-0.325433902911742	-1.21796047021955\\
-0.166427950832406	-1.13985271764912\\
-0.0212772984721446	-1.0538685255848\\
0.0865926193416984	-0.953641729425033\\
0.133275065456301	-0.83437878345467\\
0.117177063721951	-0.718619730502275\\
0.0615384745660109	-0.619305122958031\\
-0.023890767241255	-0.528236586601054\\
-0.125920352259196	-0.44348577081528\\
-0.234929250225721	-0.358702690339221\\
-0.337747374773873	-0.271096074677599\\
-0.42500490952233	-0.174848385741289\\
-0.483153087389525	-0.0670052949730876\\
-0.521824658397032	0.0517393954801681\\
-0.555568346176246	0.176002466189271\\
-0.580965393134846	0.304706565714227\\
-0.59548969932216	0.43341186778484\\
-0.595934789755774	0.560730961961262\\
-0.579349076083284	0.682367541944783\\
-0.542976269726607	0.796681168028183\\
-0.48192023028051	0.901610793058486\\
-0.378800693156139	1.01609107756565\\
-0.242114031338956	1.12837320796124\\
-0.0861105828573844	1.22804770989744\\
0.0799813639709613	1.3059252625753\\
0.243681750702025	1.35463337517742\\
0.3955967782568	1.36374686031223\\
0.523014664970328	1.32703987998776\\
0.616051646513042	1.23420482665328\\
0.636299690193864	1.12805515267803\\
0.575125722686913	1.03989380550124\\
0.458696026672357	0.959944058810537\\
0.308767528710407	0.884629803552878\\
0.149761594220362	0.806522050982455\\
0.00461091690170424	0.720537858918135\\
-0.103258958367591	0.620311062758366\\
-0.149941639973572	0.501048116788004\\
};
\addlegendentry{True curve}

\addplot [color=gray, line width=1.5pt]
  table[row sep=crcr]{%
0.0122733072808549	-1.61494779786161\\
0.0753045470308661	-1.6068993320227\\
0.13230643890902	-1.57881910216084\\
0.178114084238647	-1.53478077094656\\
0.21271103218874	-1.48148193250404\\
0.237391544386995	-1.42292779256146\\
0.255494609943319	-1.36201807244844\\
0.270106140467747	-1.30017780916862\\
0.282473285820075	-1.23784989645996\\
0.293147644227852	-1.17520986884689\\
0.301956468937787	-1.11228038772705\\
0.310243540005395	-1.04928007471272\\
0.318893506602123	-0.986328561111699\\
0.32712708542956	-0.923321234819625\\
0.334301111640158	-0.860184491676562\\
0.340544413836571	-0.796948930759719\\
0.346200735964044	-0.733658165187056\\
0.351384457143519	-0.670326940490885\\
0.355998556116153	-0.606951668677233\\
0.359907849201983	-0.543529019612782\\
0.3630517663736	-0.480063826226159\\
0.365527682236251	-0.416569064021513\\
0.367461443792031	-0.35305547844308\\
0.368833873790785	-0.289527284523514\\
0.369527235084287	-0.225988050684096\\
0.369447803971991	-0.162445083508477\\
0.368549645843299	-0.0989084145781705\\
0.366872865908379	-0.0353875251335686\\
0.364572287409382	0.0281138317444811\\
0.361827147941891	0.0915975241078551\\
0.358658712376831	0.155061498162854\\
0.354880228865579	0.218492074773339\\
0.350342032407699	0.281872827054242\\
0.345086557702587	0.345198137731786\\
0.338825400569547	0.408431933269764\\
0.331034194169084	0.471495489224126\\
0.32228432065416	0.534433194141419\\
0.31389086805082	0.597419422320117\\
0.30608798673441	0.660481534796195\\
0.297095789388963	0.723385075027918\\
0.28499350478361	0.785764957154406\\
0.271600729340809	0.847880563508383\\
0.260520151431765	0.910450011164448\\
0.246985025648622	0.972534754514308\\
0.226991447866291	1.03285035642828\\
0.210393619084698	1.09418735233223\\
0.185690977221306	1.15273215971728\\
0.149915815174163	1.20524742194917\\
0.104564193470371	1.24975523469726\\
0.0484488175748869	1.27956764108944\\
-0.0146196797704756	1.28731874613204\\
-0.0758791144547647	1.27043690236589\\
-0.128302370032466	1.23452705327934\\
-0.168828256018908	1.18558456098688\\
-0.199507585310063	1.12993841340209\\
-0.221444047649195	1.07030195972795\\
-0.238828896945421	1.00918337007038\\
-0.25330992400194	0.947312416932645\\
-0.266786903330837	0.885215025562701\\
-0.282177891965121	0.823564133795891\\
-0.295917641549925	0.761524354072472\\
-0.305013622280037	0.6986357372858\\
-0.310981650588287	0.635373603075078\\
-0.31745459532257	0.572161136161894\\
-0.326287942035999	0.509235092486609\\
-0.33631734748428	0.446488570565968\\
-0.345119659992099	0.383558178216181\\
-0.351150669700464	0.320302017182799\\
-0.35478561697595	0.256863053248259\\
-0.357653778003587	0.193384799971227\\
-0.360792278580292	0.129919338490879\\
-0.364097592024437	0.0664623460486003\\
-0.36709916248155	0.00299026114842968\\
-0.369343450477018	-0.0605131100863078\\
-0.370479982397387	-0.124045962076262\\
-0.370478240197162	-0.187588978873926\\
-0.369659948389828	-0.2511267265937\\
-0.368566466903158	-0.314660334117763\\
-0.367382470802894	-0.37819231929073\\
-0.365819321962486	-0.441716106587193\\
-0.363229797037992	-0.505206336917921\\
-0.359223336691215	-0.568622921990543\\
-0.354345737191754	-0.631978458527663\\
-0.349412010872846	-0.695329648977359\\
-0.344373669112038	-0.75867260516891\\
-0.338591695013489	-0.821952015424594\\
-0.331802737950302	-0.885131324132253\\
-0.324034367375478	-0.948197697148273\\
-0.315622551819222	-1.01118147558233\\
-0.307033669133691	-1.07414135233728\\
-0.298359144115146	-1.13708948656289\\
-0.289193262704417	-1.19996795350308\\
-0.27959849200064	-1.26278240535873\\
-0.264804293551827	-1.32457922306838\\
-0.247752248288461	-1.38579149911755\\
-0.227405610799124	-1.44598891874382\\
-0.20064784656047	-1.5036234313186\\
-0.160803046236957	-1.55312198557994\\
-0.111214418980975	-1.59285463001308\\
-0.0512612350298965	-1.61391005023951\\
0.0122733072808549	-1.61494779786161\\
};
\addlegendentry{Initial guess}

\addplot [color=black, line width=1.5pt]
  table[row sep=crcr]{%
-0.137055455815303	-1.64470226397497\\
-0.0529434172271665	-1.64142689286902\\
0.0393168936187488	-1.62687553182872\\
0.121083926003523	-1.57673243678822\\
0.189248656547826	-1.50291633802197\\
0.253581561348028	-1.43263612973397\\
0.324354778617567	-1.37249958734053\\
0.392754699851265	-1.32402455505709\\
0.45843909308069	-1.27294774167647\\
0.516125273941028	-1.20520789145022\\
0.551814637425638	-1.11793418925221\\
0.563173847376657	-1.03493680694231\\
0.56328082834659	-0.95073220198696\\
0.561438242001149	-0.8574997469925\\
0.565125173392965	-0.749936095890265\\
0.571843578194094	-0.635777291960067\\
0.563770603675999	-0.513303165016059\\
0.523870936166608	-0.400170192952606\\
0.463298346367883	-0.307806603488396\\
0.405637774130739	-0.235439498339572\\
0.35376913152548	-0.166781657560857\\
0.308338261403267	-0.0953001671535129\\
0.265967354838928	-0.0160852628595135\\
0.226747834902041	0.0663843491431273\\
0.184976959633269	0.150319579691641\\
0.137431901410485	0.229535118319092\\
0.0821847764925601	0.30353314899081\\
0.0277401407719371	0.368142978290563\\
-0.0237982651065853	0.430451484841473\\
-0.0658534349268723	0.491197686362474\\
-0.0978554259216416	0.556848872842953\\
-0.11414319058874	0.625910343096606\\
-0.111158948205298	0.697652338642998\\
-0.0865371457916102	0.76595726258076\\
-0.0469400971352654	0.81983928516409\\
0.00293500585845091	0.861604738422561\\
0.0558084783566562	0.891432644090821\\
0.118881460838802	0.915065105374292\\
0.177833405456798	0.92901943145484\\
0.23918915883029	0.939013751772845\\
0.290463721076705	0.946579485721212\\
0.344393384951301	0.954203362530445\\
0.392164904496254	0.961625286890615\\
0.457666985265373	0.977495809277965\\
0.501470207833091	0.993868144065148\\
0.5799497495688	1.03378598010436\\
0.62920182173784	1.12808442021001\\
0.564582243273621	1.31769715082001\\
0.481500494640982	1.32974407055995\\
0.426261718064856	1.33839988379953\\
0.364424491966809	1.34507631389916\\
0.26823851058225	1.35156625527738\\
0.12922472286853	1.34244395116392\\
0.0535536948418623	1.28962944467141\\
-0.0291012715367924	1.22176568208047\\
-0.135151970131844	1.17904289941093\\
-0.219432560625033	1.16070406127821\\
-0.302498297873301	1.12014065859151\\
-0.342434643280267	1.0652203241597\\
-0.360820045284729	1.01555416700143\\
-0.38161140376294	0.956298063384535\\
-0.425034689158147	0.893113293831372\\
-0.484271479999175	0.847982096176667\\
-0.525666682683243	0.822129929379117\\
-0.566844035581275	0.788002494980382\\
-0.597427386732497	0.731720086219255\\
-0.594939406498209	0.629648893860952\\
-0.577042997156975	0.535522179281208\\
-0.569790751894312	0.407725859744351\\
-0.577013525176406	0.286683018975134\\
-0.569906963702629	0.155041455020797\\
-0.526651708685133	0.0361553893123887\\
-0.448946594238679	-0.0707073462493093\\
-0.370344971450132	-0.160383073029636\\
-0.292965748568815	-0.263646865122831\\
-0.231787137222139	-0.37657041090048\\
-0.178419619528483	-0.508667923275861\\
-0.130278481270882	-0.63323545216383\\
-0.082530118218802	-0.751766974133133\\
-0.0477917426021225	-0.845226317234882\\
-0.0270646426447088	-0.924383782651552\\
-0.017607041862556	-0.987969858303597\\
-0.0162932508218875	-1.05458031791468\\
-0.0275707936896662	-1.12118995289855\\
-0.0614870225390689	-1.19431110402005\\
-0.119609692268831	-1.25482720526498\\
-0.21732705777679	-1.30293549848083\\
-0.33272189519266	-1.32535845396207\\
-0.453097123692693	-1.32826564593813\\
-0.573485795358524	-1.35550772127413\\
-0.661371378915472	-1.4620465353987\\
-0.63834316219768	-1.54623321326203\\
-0.590574094007759	-1.60544251165222\\
-0.544295461188492	-1.64747574372301\\
-0.496387330433575	-1.68262599044326\\
-0.433820780534745	-1.70705087044812\\
-0.359653714308438	-1.70242934483034\\
-0.292494530169302	-1.67887404387462\\
-0.227250060242447	-1.65591740916184\\
-0.191828112058339	-1.651392340458\\
-0.137055455815303	-1.64470226397497\\
};
\addlegendentry{Reconstruction}

\end{axis}
\end{tikzpicture}%

==> Dir-source-obstacle/source_obstacle6.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=1.5in,
height=1.5in,
at={(0.867in,0.478in)},
scale only axis,
point meta min=0.261666496529607,
point meta max=12.9134088621672,
axis on top,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=-3,
xmax=3,
xtick={-3,-1.5,0,1.5,3},
tick align=outside,
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymin=-3,
ymax=4,
ytick={-3,-1.5,0,1.5,3},
axis background/.style={fill=white},
title style={font=\normalfont},
title={Source and obstacle},
%legend style={legend cell align=left, align=left, draw=black},
legend style={legend cell align=left, align=left, draw=black, font=\tiny, at={(1,0.7)}, anchor=south east},
colormap/hot2,
colorbar,
colorbar style={separate axis lines, every outer x axis line/.append style={black}, every x tick label/.append style={font=\color{black}}, every x tick/.append style={black}, every outer y axis line/.append style={black}, every y tick label/.append style={font=\color{black}}, every y tick/.append style={black}}
]
\addplot [forget plot] graphics [xmin=-2.03571428571429, xmax=-1.46428571428571, ymin=-1.54838709677419, ymax=1.54838709677419] {Dir-source-obstacle/source_obstacle6-1.png};
\addplot [forget plot] graphics [xmin=1.46428571428571, xmax=2.03571428571429, ymin=-1.54838709677419, ymax=1.54838709677419] {Dir-source-obstacle/source_obstacle6-2.png};
\addplot [color=orange, line width=1.5pt]
  table[row sep=crcr]{%
-0.149941639973572	0.501048116788004\\
-0.133843792338541	0.385289063835608\\
-0.0782051586544083	0.285974456291364\\
0.00722405612213784	0.194905919934387\\
0.10925366094537	0.110155104148614\\
0.218262542944971	0.0253720236725542\\
0.321080681214414	-0.0622345919890673\\
0.408338203540294	-0.158482280925378\\
0.466486393236096	-0.266325371693579\\
0.505157952343543	-0.385070062146835\\
0.538901652772338	-0.509333132855938\\
0.564298688438677	-0.638037232380894\\
0.578823283965763	-0.766742534451507\\
0.579268435191686	-0.894061628627929\\
0.562682703126582	-1.01569820861145\\
0.526309907313376	-1.13001183469485\\
0.465253860278564	-1.23494145972515\\
0.362134329376925	-1.34942174423232\\
0.225447661988721	-1.4617038746279\\
0.0694442188187118	-1.56137837656411\\
-0.0966477333142413	-1.63925592924197\\
-0.260348114558843	-1.68796404184409\\
-0.412263147945908	-1.69707752697889\\
-0.53968102831698	-1.66037054665443\\
-0.632718016899188	-1.56753549331994\\
-0.652966052607406	-1.4613858193447\\
-0.591792094332252	-1.37322447216791\\
-0.475362387336835	-1.2932747254772\\
-0.325433902911742	-1.21796047021955\\
-0.166427950832406	-1.13985271764912\\
-0.0212772984721446	-1.0538685255848\\
0.0865926193416984	-0.953641729425033\\
0.133275065456301	-0.83437878345467\\
0.117177063721951	-0.718619730502275\\
0.0615384745660109	-0.619305122958031\\
-0.023890767241255	-0.528236586601054\\
-0.125920352259196	-0.44348577081528\\
-0.234929250225721	-0.358702690339221\\
-0.337747374773873	-0.271096074677599\\
-0.42500490952233	-0.174848385741289\\
-0.483153087389525	-0.0670052949730876\\
-0.521824658397032	0.0517393954801681\\
-0.555568346176246	0.176002466189271\\
-0.580965393134846	0.304706565714227\\
-0.59548969932216	0.43341186778484\\
-0.595934789755774	0.560730961961262\\
-0.579349076083284	0.682367541944783\\
-0.542976269726607	0.796681168028183\\
-0.48192023028051	0.901610793058486\\
-0.378800693156139	1.01609107756565\\
-0.242114031338956	1.12837320796124\\
-0.0861105828573844	1.22804770989744\\
0.0799813639709613	1.3059252625753\\
0.243681750702025	1.35463337517742\\
0.3955967782568	1.36374686031223\\
0.523014664970328	1.32703987998776\\
0.616051646513042	1.23420482665328\\
0.636299690193864	1.12805515267803\\
0.575125722686913	1.03989380550124\\
0.458696026672357	0.959944058810537\\
0.308767528710407	0.884629803552878\\
0.149761594220362	0.806522050982455\\
0.00461091690170424	0.720537858918135\\
-0.103258958367591	0.620311062758366\\
-0.149941639973572	0.501048116788004\\
};
\addlegendentry{True curve}

\addplot [color=gray, line width=1.5pt]
  table[row sep=crcr]{%
0.0122733072808549	-1.61494779786161\\
0.0753045470308661	-1.6068993320227\\
0.13230643890902	-1.57881910216084\\
0.178114084238647	-1.53478077094656\\
0.21271103218874	-1.48148193250404\\
0.237391544386995	-1.42292779256146\\
0.255494609943319	-1.36201807244844\\
0.270106140467747	-1.30017780916862\\
0.282473285820075	-1.23784989645996\\
0.293147644227852	-1.17520986884689\\
0.301956468937787	-1.11228038772705\\
0.310243540005395	-1.04928007471272\\
0.318893506602123	-0.986328561111699\\
0.32712708542956	-0.923321234819625\\
0.334301111640158	-0.860184491676562\\
0.340544413836571	-0.796948930759719\\
0.346200735964044	-0.733658165187056\\
0.351384457143519	-0.670326940490885\\
0.355998556116153	-0.606951668677233\\
0.359907849201983	-0.543529019612782\\
0.3630517663736	-0.480063826226159\\
0.365527682236251	-0.416569064021513\\
0.367461443792031	-0.35305547844308\\
0.368833873790785	-0.289527284523514\\
0.369527235084287	-0.225988050684096\\
0.369447803971991	-0.162445083508477\\
0.368549645843299	-0.0989084145781705\\
0.366872865908379	-0.0353875251335686\\
0.364572287409382	0.0281138317444811\\
0.361827147941891	0.0915975241078551\\
0.358658712376831	0.155061498162854\\
0.354880228865579	0.218492074773339\\
0.350342032407699	0.281872827054242\\
0.345086557702587	0.345198137731786\\
0.338825400569547	0.408431933269764\\
0.331034194169084	0.471495489224126\\
0.32228432065416	0.534433194141419\\
0.31389086805082	0.597419422320117\\
0.30608798673441	0.660481534796195\\
0.297095789388963	0.723385075027918\\
0.28499350478361	0.785764957154406\\
0.271600729340809	0.847880563508383\\
0.260520151431765	0.910450011164448\\
0.246985025648622	0.972534754514308\\
0.226991447866291	1.03285035642828\\
0.210393619084698	1.09418735233223\\
0.185690977221306	1.15273215971728\\
0.149915815174163	1.20524742194917\\
0.104564193470371	1.24975523469726\\
0.0484488175748869	1.27956764108944\\
-0.0146196797704756	1.28731874613204\\
-0.0758791144547647	1.27043690236589\\
-0.128302370032466	1.23452705327934\\
-0.168828256018908	1.18558456098688\\
-0.199507585310063	1.12993841340209\\
-0.221444047649195	1.07030195972795\\
-0.238828896945421	1.00918337007038\\
-0.25330992400194	0.947312416932645\\
-0.266786903330837	0.885215025562701\\
-0.282177891965121	0.823564133795891\\
-0.295917641549925	0.761524354072472\\
-0.305013622280037	0.6986357372858\\
-0.310981650588287	0.635373603075078\\
-0.31745459532257	0.572161136161894\\
-0.326287942035999	0.509235092486609\\
-0.33631734748428	0.446488570565968\\
-0.345119659992099	0.383558178216181\\
-0.351150669700464	0.320302017182799\\
-0.35478561697595	0.256863053248259\\
-0.357653778003587	0.193384799971227\\
-0.360792278580292	0.129919338490879\\
-0.364097592024437	0.0664623460486003\\
-0.36709916248155	0.00299026114842968\\
-0.369343450477018	-0.0605131100863078\\
-0.370479982397387	-0.124045962076262\\
-0.370478240197162	-0.187588978873926\\
-0.369659948389828	-0.2511267265937\\
-0.368566466903158	-0.314660334117763\\
-0.367382470802894	-0.37819231929073\\
-0.365819321962486	-0.441716106587193\\
-0.363229797037992	-0.505206336917921\\
-0.359223336691215	-0.568622921990543\\
-0.354345737191754	-0.631978458527663\\
-0.349412010872846	-0.695329648977359\\
-0.344373669112038	-0.75867260516891\\
-0.338591695013489	-0.821952015424594\\
-0.331802737950302	-0.885131324132253\\
-0.324034367375478	-0.948197697148273\\
-0.315622551819222	-1.01118147558233\\
-0.307033669133691	-1.07414135233728\\
-0.298359144115146	-1.13708948656289\\
-0.289193262704417	-1.19996795350308\\
-0.27959849200064	-1.26278240535873\\
-0.264804293551827	-1.32457922306838\\
-0.247752248288461	-1.38579149911755\\
-0.227405610799124	-1.44598891874382\\
-0.20064784656047	-1.5036234313186\\
-0.160803046236957	-1.55312198557994\\
-0.111214418980975	-1.59285463001308\\
-0.0512612350298965	-1.61391005023951\\
0.0122733072808549	-1.61494779786161\\
};
\addlegendentry{Initial guess}

\addplot [color=black, line width=1.5pt]
  table[row sep=crcr]{%
-0.003016823787138	-1.59975768866901\\
0.110099180307909	-1.55031205169291\\
0.212570220765322	-1.50197140950647\\
0.278748593834767	-1.44869485563883\\
0.335612199808092	-1.38105938417203\\
0.379397249591442	-1.32247118247132\\
0.425936420507708	-1.26540704706963\\
0.469050153498441	-1.21748477064912\\
0.516348584805177	-1.16550133779098\\
0.557368554684639	-1.1105648511489\\
0.589008903787776	-1.03771584113544\\
0.596477008177663	-0.966797508643942\\
0.58678600427604	-0.898053645016472\\
0.566427033750685	-0.82236991434226\\
0.548091427111232	-0.724850156946577\\
0.547973060192714	-0.616001827900265\\
0.557277133322228	-0.49914420041704\\
0.540056267677944	-0.385322714621589\\
0.483932189462489	-0.290828670286303\\
0.425962041495603	-0.230149482110708\\
0.373926843831157	-0.180800293925357\\
0.323356476868906	-0.129324201343325\\
0.271577429758707	-0.0686873012520933\\
0.222469527208651	-0.000680323814929567\\
0.176695817903157	0.0701012319926545\\
0.131555282111414	0.141153337449735\\
0.085560716189554	0.211286543972732\\
0.0399869340306451	0.280563843547856\\
-0.000769126263908818	0.348268178315944\\
-0.0334158223462209	0.415914463996549\\
-0.0549906429696636	0.48368594400727\\
-0.0631159044179719	0.550298460675507\\
-0.0562534871626557	0.617701690811196\\
-0.0353179716986061	0.67802873039452\\
-0.000463981666878204	0.733654847784688\\
0.0392832413156334	0.776832236741707\\
0.0905783403426434	0.818232701056283\\
0.143703751909943	0.850821195112882\\
0.205810413536872	0.879315957324764\\
0.258010508666821	0.898890313939135\\
0.315188702021157	0.918219185992948\\
0.359338549796473	0.931564158133977\\
0.414606095563798	0.947213599240215\\
0.462681837156871	0.961892145386777\\
0.513232743178917	0.983315315335044\\
0.568884829539868	1.00506096699034\\
0.62027695469827	1.21482203879172\\
0.60866450394752	1.27575291191864\\
0.381622235148417	1.35666109721811\\
0.347330989893445	1.37302691034562\\
0.320589492149972	1.38154922936614\\
0.271801742897361	1.38463554911428\\
0.220946379677073	1.36740783686596\\
0.159453184472982	1.31541629616534\\
0.0396781106836049	1.24615453882332\\
-0.0628678747878493	1.22774113071671\\
-0.155502493740789	1.21151247161664\\
-0.215473755353387	1.18612864899312\\
-0.259668287953593	1.15042122971856\\
-0.29445530297554	1.09592812525836\\
-0.323550024651566	1.02237348996731\\
-0.36356485144663	0.953976846518261\\
-0.433030294753316	0.895721382411532\\
-0.48495124494914	0.867684998874094\\
-0.527823425464779	0.843711756098114\\
-0.578895602480457	0.792171957510417\\
-0.594292735434631	0.711666113543468\\
-0.577598966933144	0.623808186306372\\
-0.560970226561983	0.522370990269143\\
-0.566894951579642	0.416196663613815\\
-0.588802828332015	0.296422216046327\\
-0.586828524179823	0.179394502485458\\
-0.534932427362436	0.0563784945823646\\
-0.459580092081427	-0.0467440307588161\\
-0.381955656819244	-0.151824147856899\\
-0.312821137244099	-0.267823122572448\\
-0.248415951604844	-0.402603009726384\\
-0.181417051391753	-0.539507042068511\\
-0.109591924557318	-0.668299907041415\\
-0.0472963577727909	-0.772624680357536\\
-0.0052593069967769	-0.856696101822724\\
0.021774135569685	-0.924740779424787\\
0.042376155800356	-0.994289653930169\\
0.052007638331305	-1.06961568057083\\
0.0387276101308649	-1.16044254399827\\
-0.00461508329592813	-1.23730358589052\\
-0.109098280127266	-1.30383338901183\\
-0.228479598549582	-1.32694480099228\\
-0.396639052452272	-1.32435867240707\\
-0.49818200141737	-1.32635229728353\\
-0.627475798604177	-1.39394191934667\\
-0.652419433782936	-1.47138254312321\\
-0.594803378568887	-1.62530393785283\\
-0.535496537356052	-1.66488649245886\\
-0.471197769940781	-1.6875465804379\\
-0.406068054336531	-1.69863902294381\\
-0.282079778684305	-1.69873115739137\\
-0.191778170101687	-1.67407543364198\\
-0.134302734819771	-1.64567551896757\\
-0.0977022643558427	-1.63499563983008\\
-0.003016823787138	-1.59975768866901\\
};
\addlegendentry{Reconstruction}

\end{axis}
\end{tikzpicture}%
